A Rapid Algorithm for Beam Illumination Patterns and Hopping Time Plan

Beam hopping (BH) is a satellite communications technique in which sets of beams are sequentially illuminated over a defined time interval. Geographically varying the duty cycle of satellite transmission allows for reduced resource wastage as satellite capacity is matched to non-uniform user demands. Total feasible active beam combinations is given by $2^n$ for $n$ beams. With in service satellite systems operating in excess of 100 beams, complete enumeration of optimum illumination patterns is not tractable. Developing efficient optimization methods which minimize resource wastage is essential to realising the benefits of modern BH systems. We present a computationally efficient pattern generation method which uses the binary logarithm to decompose beam demands into common powers of two. This method is shown to produce feasible patterns within 0.047 and 0.31 seconds for systems using 49 and 132 beams respectively and within 19.109 seconds for a 1085 beam system. When averaged across all testing configurations, this method reduced capacity error by 94% compared to a conventional even data distribution. To facilitate algorithm comparison, two integer linear programming formulations are developed. Even though they can only solve problems of modest sizes to proven optimality, they provide valuable insights in the optimality gap for our proposed heuristic approach.

==> litReview.tex <==
Most previous work in the literature of BH scheduling optimization are   heuristic or meta-heuristic approaches such as the Genetic Algorithm (GA), see, for example \cite{angeletti2006beam} and \cite{anzalchi2010beam}, the latter also considered applying  GA, Variable Neighbour Search (VNS), and Iterated Local Search (ILS) sequentially for finidng the optimal BHTP, power plan, and frequency plan. Other constraints considered include: Constraints considered include an upper bound on the number of simultaneously illuminated beams at any time slot, (i.e., $N_{MAX}$), an upper bound on total processed bandwidth, a lower bound on beam capacity, an UB on HPAs' output RF-power and the total DC-power budget. 
% 
Iterative or incremental heuristic allocation has been applied in, e.g., \cite{alberti2010system}. \cite{alegre2012offered}  considered time allocation and power allocation to beams. Two iterative algorithms are proposed: an Iterative Minimal Co-channel Interference (minCCI) Algorithm and an Iterative SINR Maximization (maxSINR), both are sequential construction algorithms however with different objectives used.  
% 
In \cite{lei2011multibeam} When co-channel interference is considered, an heuristic iterative approach is implemented where in the first instance, the problem of allocating carrier (frequency bandwidth) or time on a per-beam basis is solved by finding the argument that provides the maximum Rayleigh quotient for each beam, subject to an upper bound on the total power. Then, the power to be allocated to the selected carriers from the power constraint will be calculated. When co-channel interference is not considered, the optimization problems are formulated as convex programming problems, and Lagrangean relaxation is used for finding the optimal solution.  
 

\cite{Kyrgiazos2013} considered beams of two sizes: small beams over areas with high traffic demands and large beams for areas with low traffic demands. kMeans is used for clustering grid points into clusters. Demand aggregation is performed. BH pattern is found by solving a binary linear programming problem, with max number of illuminated beams bounded from above, and interference eliminated by a set packing constraint. The objective coefficient considers the beam dwell time (that is calculated as a log function of capacity over requested demand). {\bf come back to this later - a bit more details} 

% \cite{Sormunen2017} System level modeling of beam hopping for multi-spot beam satellite systems

\cite{Shi2017} Joint power and bandwidth allocation for beam-hopping user downlinks in smart gateway multibeam satellite systems

\cite{Tani2018} Overlapping clustering for beam-hopping systems

\cite{Rohde:2018} Beam-hopping systems for next generation satellite communication systems

\cite{Kibria2019} Precoded Cluster Hopping in Multi-Beam High Throughput Satellite Systems

\cite{Koosha2019} A hybrid beam hopping design for non-uniform traffic in HTS networks

\cite{Zhang2019} Dynamic beam hopping for DVB-S2X satellite: A multi-objective deep reinforcement learning approach

\cite{Wang2019} Resource allocation for beam-hopping user downlinks in multi-beam satellite system

\cite{Hu2019} Deep reinforcement learning-based beam Hopping algorithm in multibeam satellite systems

\cite{Wang2019a} A Flexible Resource Allocation Algorithm in Full Bandwidth Beam Hopping Satellite Systems

\cite{hu2020dynamic} Dynamic beam hopping method based on multi-objective deep reinforcement learning for next generation satellite broadband systems

\cite{lei2020beam} Beam illumination pattern design in satellite networks: Learning and optimization for efficient beam hopping

\cite{Zhang2020} Design of next generation high throughput satellite communication system based on beam-hopping

\cite{Shi2020} Resource Allocation in Beam Hopping Communication Satellite System


\cite{Lei2020} Deep Learning for Beam Hopping in Multibeam Satellite Systems

\cite{Zhao2021} Beam Hopping Resource Allocation for Uneven Traffic Distribution in HTS System
